What's in your Head? Emergent Behaviour in Multi-Task Transformer Models

The primary paradigm for multi-task training in natural language processing is to represent the input with a shared pre-trained language model, and add a small, thin network (head) per task. Given an input, a target head is the head that is selected for outputting the final prediction. In this work, we examine the behaviour of non-target heads, that is, the output of heads when given input that belongs to a different task than the one they were trained for. We find that non-target heads exhibit emergent behaviour, which may either explain the target task, or generalize beyond their original task. For example, in a numerical reasoning task, a span extraction head extracts from the input the arguments to a computation that results in a number generated by a target generative head. In addition, a summarization head that is trained with a target question answering head, outputs query-based summaries when given a question and a context from which the answer is to be extracted. This emergent behaviour suggests that multi-task training leads to non-trivial extrapolation of skills, which can be harnessed for interpretability and generalization.

==> 093_example_sf.tex <==

\section{Example Emergent Supporting Facts}
\label{sec:example_emergent_sf}

Examples are provided in Table~\ref{table:example_sf}.

\begin{table*}[t]
    \centering
    \footnotesize
    \begin{tabular}{p{6cm}|p{7.5cm}}
          Question & Top-5 extracted spans \\ \toprule
          Can Stenocereus and Pachypodium both include tree like plants? (\nl{yes}) & 
          \begin{enumerate}[leftmargin=*,topsep=0pt,itemsep=0pt,parsep=0pt]
              \item Pachypodium
              \item Stenocereus
              \item eus
              \item Stenocereus (Gk. stenos, narrow, L. cereus, candle) is a genus of columnar or tree-like
              \item Pachypodium is a genus of succulent spine-bearing trees
          \end{enumerate}
          \\ \hline
          Were Goo Goo Dolls and Echosmith formed in the same city? (\nl{no}) & 
          \begin{enumerate}[leftmargin=*,topsep=0pt,itemsep=0pt,parsep=0pt]
              \item Goo Goo Dolls
              \item Goo Goo Dolls are an American rock band formed in 1985 in Buffalo, New York
              \item Echosmith is an American, Corporate indie pop band formed in February 2009 in Chino, California
              \item New York
              \item Chino, California
          \end{enumerate}
          \\ \hline
          Is the building located at 200 West Street taller than the one at 888 7th Avenue? (\nl{yes}) & 
          \begin{enumerate}[leftmargin=*,topsep=0pt,itemsep=0pt,parsep=0pt]
              \item building
              \item building is a 749 ft , 44-story building
              \item The building
              \item The building is a 749 ft , 44-story building
              \item 888 7th Avenue is a 628 ft (191m) tall
          \end{enumerate}
          \\ \hline
    \end{tabular}
    \caption{Example questions from \hotpotqa{} and the extracted spans by the \reader{} model.}
    \label{table:example_sf}
\end{table*}

